Agent-R: Training Language Model Agents to Reflect via Iterative Self-Training

Large Language Models (LLMs) agents are increasingly pivotal for addressing complex tasks in interactive environments. Existing work mainly focuses on enhancing performance through behavior cloning from stronger experts, yet such approaches often falter in real-world applications, mainly due to the inability to recover from errors. However, step-level critique data is difficult and expensive to collect. Automating and dynamically constructing self-critique datasets is thus crucial to empowering models with intelligent agent capabilities. In this work, we propose an iterative self-training framework, Agent-R, that enables language Agent to Reflect on the fly. Unlike traditional methods that reward or penalize actions based on correctness, Agent-R leverages MCTS to construct training data that recover correct trajectories from erroneous ones. A key challenge of agent reflection lies in the necessity for timely revision rather than waiting until the end of a rollout. To address this, we introduce a model-guided critique construction mechanism: the actor model identifies the first error step (within its current capability) in a failed trajectory. Starting from it, we splice it with the adjacent correct path, which shares the same parent node in the tree. This strategy enables the model to learn reflection based on its current policy, therefore yielding better learning efficiency. To further explore the scalability of this self-improvement paradigm, we investigate iterative refinement of both error correction capabilities and dataset construction. Our findings demonstrate that Agent-R continuously improves the model's ability to recover from errors and enables timely error correction. Experiments on three interactive environments show that Agent-R effectively equips agents to correct erroneous actions while avoiding loops, achieving superior performance compared to baseline methods (+5.59%).

==> table/revision_discard.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{lcccc}
    \toprule
        \textbf{Method} & \textbf{WebShop} & \textbf{SciWorld} & \textbf{TextCraft} & \textbf{Average} \\ 
    \midrule
        AgentLM-7B & 32.14 & 0.00 & 0.00 & 10.71  \\ 
        AgentLM-13B & 34.42 & 0.00 & 0.00 & 11.47  \\ 
        AgentEvol & 27.36 & 0.88 & 0.00 & 9.41 \\ 
        GPT-4o & 19.82  & 43.00  & 6.76  & 23.19   \\ 
    \midrule
    \rowcolor[gray]{0.95}\multicolumn{5}{c}{\textit{Llama-3.1-8B}} \\
        w/ Optimal & 30.94 & 1.38  & 0.00 & 10.77  \\ 
        w/ Optimal+ & 21.23 & 2.51  & 0.00 & 7.91  \\ 
        w/ ETO & 35.76 & 1.15  & 0.00 & 12.30  \\ 
    \midrule
    \rowcolor[gray]{0.95}\multicolumn{5}{c}{\textit{Llama-3.1-8B w/ Direct-Revision + Good Trajectories}} \\
        \# Iter1 & 38.52 & 18.90 & 8.11 & 21.84  \\ 
        \# Iter2 & 41.05 & 22.00 & 19.73 & 27.59  \\ 
        \# Iter3 & \textbf{44.03} & \underline{26.50} & \underline{24.32} & \underline{31.62} \\ 
    \midrule
    \rowcolor[gray]{0.95}\multicolumn{5}{c}{\textit{Llama-3.1-8B w/ Trajectories from \method}} \\
        \# Iter1 & 40.80 & 24.80 & 12.16 & 25.92 \\ 
        \# Iter2 & \underline{41.94} & \underline{26.50} & 20.27 & 29.57 \\ 
        \# Iter3 & \textbf{44.03} & \textbf{29.54} & \textbf{27.03} & \textbf{33.53} \\ 
    \bottomrule
    \end{tabular}
    \caption{The revision results of different methods. \textit{w/ Optimal+} means the golden trajectories for training Llama-3.1-8B are generated from GPT-4o.\ysy{need to randomly concat.}
  }
  \label{tab:revision}
\end{table}
